Environment Design for Inverse Reinforcement Learning

Learning a reward function from demonstrations suffers from low sample-efficiency. Even with abundant data, current inverse reinforcement learning methods that focus on learning from a single environment can fail to handle slight changes in the environment dynamics. We tackle these challenges through adaptive environment design. In our framework, the learner repeatedly interacts with the expert, with the former selecting environments to identify the reward function as quickly as possible from the expert's demonstrations in said environments. This results in improvements in both sample-efficiency and robustness, as we show experimentally, for both exact and approximate inference.

==> figures/mazes/10_steps_additional/plot_seed_1.tex <==
\begin{figure}[t]

\centering
        
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/1_env.png}};
            \draw (0, 1.3) node {\tiny Sampled mazes (DR)};
            \draw (-1.3, 0) node {\tiny 1};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny DR-BIRL};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_1/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Coordinate-wise avg};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_1/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Coordinate-wise max};
        \end{tikzpicture}
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/2_env.png}};
            \draw (-1.3, 0) node {\tiny 2};
         \end{tikzpicture}
          \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/2_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_1/2_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_1/2_rounded_scaled_mean.png} 
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/3_env.png}};
            \draw (-1.3, 0) node {\tiny 3};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/3_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_1/3_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_1/3_rounded_scaled_mean.png}
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/4_env.png}};
            \draw (-1.3, 0) node {\tiny 4};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/4_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_1/4_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_1/4_rounded_scaled_mean.png} 
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/5_env.png}};
            \draw (-1.3, 0) node {\tiny 5};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/5_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_1/5_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_1/5_rounded_scaled_mean.png}
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/6_env.png}};
            \draw (-1.3, 0) node {\tiny 6};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/6_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_1/6_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_1/6_rounded_scaled_mean.png} 
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/7_env.png}};
            \draw (-1.3, 0) node {\tiny 7};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/7_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_1/7_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_1/7_rounded_scaled_mean.png} 
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/8_env.png}};
            \draw (-1.3, 0) node {\tiny 8};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_1/8_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_1/8_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_1/8_rounded_scaled_mean.png}  
            
     \caption*{Run 2} 
     \label{fig:dr_additional_experiment_seed_1}
\end{figure}

==> figures/mazes/10_steps_additional/plot_seed_2.tex <==
\begin{figure}[t]

\centering
        
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/1_env.png}};
            \draw (0, 1.3) node {\tiny Sampled mazes (DR)};
            \draw (-1.3, 0) node {\tiny 1};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny DR-BIRL};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_2/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Coordinate-wise avg};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_2/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Coordinate-wise max};
        \end{tikzpicture}
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/2_env.png}};
            \draw (-1.3, 0) node {\tiny 2};
         \end{tikzpicture}
          \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/2_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_2/2_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_2/2_rounded_scaled_mean.png} 
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/3_env.png}};
            \draw (-1.3, 0) node {\tiny 3};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/3_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_2/3_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_2/3_rounded_scaled_mean.png}
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/4_env.png}};
            \draw (-1.3, 0) node {\tiny 4};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/4_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_2/4_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_2/4_rounded_scaled_mean.png} 
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/5_env.png}};
            \draw (-1.3, 0) node {\tiny 5};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/5_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_2/5_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_2/5_rounded_scaled_mean.png}
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/6_env.png}};
            \draw (-1.3, 0) node {\tiny 6};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/6_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_2/6_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_2/6_rounded_scaled_mean.png} 
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/7_env.png}};
            \draw (-1.3, 0) node {\tiny 7};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/7_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_2/7_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_2/7_rounded_scaled_mean.png} 
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/8_env.png}};
            \draw (-1.3, 0) node {\tiny 8};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_2/8_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_2/8_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_2/8_rounded_scaled_mean.png}  
            
     \caption*{Run 3} 
     \label{fig:dr_additional_experiment_seed_2}
\end{figure}

==> figures/mazes/10_steps_additional/plot_seed_3.tex <==
\begin{figure}[t]

\centering
        
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/1_env.png}};
            \draw (0, 1.3) node {\tiny Sampled mazes (DR)};
            \draw (-1.3, 0) node {\tiny 1};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny DR-BIRL};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_3/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Coordinate-wise avg};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_3/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Coordinate-wise max};
        \end{tikzpicture}
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/2_env.png}};
            \draw (-1.3, 0) node {\tiny 2};
         \end{tikzpicture}
          \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/2_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_3/2_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_3/2_rounded_scaled_mean.png} 
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/3_env.png}};
            \draw (-1.3, 0) node {\tiny 3};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/3_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_3/3_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_3/3_rounded_scaled_mean.png}
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/4_env.png}};
            \draw (-1.3, 0) node {\tiny 4};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/4_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_3/4_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_3/4_rounded_scaled_mean.png} 
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/5_env.png}};
            \draw (-1.3, 0) node {\tiny 5};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/5_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_3/5_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_3/5_rounded_scaled_mean.png}
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/6_env.png}};
            \draw (-1.3, 0) node {\tiny 6};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/6_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_3/6_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_3/6_rounded_scaled_mean.png} 
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/7_env.png}};
            \draw (-1.3, 0) node {\tiny 7};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/7_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_3/7_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_3/7_rounded_scaled_mean.png} 
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/8_env.png}};
            \draw (-1.3, 0) node {\tiny 8};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_3/8_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_3/8_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_3/8_rounded_scaled_mean.png}  
            
     \caption*{Run 4} 
     \label{fig:dr_additional_experiment_seed_3}
\end{figure}

==> figures/mazes/10_steps_additional/plot_seed_4.tex <==
\begin{figure}[t]

\centering
        
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/1_env.png}};
            \draw (0, 1.3) node {\tiny Sampled mazes (DR)};
            \draw (-1.3, 0) node {\tiny 1};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny DR-BIRL};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_4/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Coordinate-wise avg};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_4/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Coordinate-wise max};
        \end{tikzpicture}
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/2_env.png}};
            \draw (-1.3, 0) node {\tiny 2};
         \end{tikzpicture}
          \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/2_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_4/2_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_4/2_rounded_scaled_mean.png} 
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/3_env.png}};
            \draw (-1.3, 0) node {\tiny 3};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/3_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_4/3_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_4/3_rounded_scaled_mean.png}
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/4_env.png}};
            \draw (-1.3, 0) node {\tiny 4};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/4_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_4/4_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_4/4_rounded_scaled_mean.png} 
        %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/5_env.png}};
            \draw (-1.3, 0) node {\tiny 5};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/5_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_4/5_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_4/5_rounded_scaled_mean.png}
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/6_env.png}};
            \draw (-1.3, 0) node {\tiny 6};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/6_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_4/6_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_4/6_rounded_scaled_mean.png} 
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/7_env.png}};
            \draw (-1.3, 0) node {\tiny 7};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/7_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_4/7_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_4/7_rounded_scaled_mean.png} 
         %
        \\
        %
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/8_env.png}};
            \draw (-1.3, 0) node {\tiny 8};
         \end{tikzpicture}
         \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr/seed_4/8_rounded_scaled_mean.png} 
           \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_mean/seed_4/8_rounded_scaled_mean.png} 
            \includegraphics[height=0.14\textwidth]{figures/mazes/10_steps_additional/dr_coord_max/seed_4/8_rounded_scaled_mean.png}  
            
     \caption*{Run 5} 
     \label{fig:dr_additional_experiment_seed_4}
\end{figure}

==> figures/mazes/maze_exp_2/maze_figure_2.tex <==
\begin{figure}[H]
     \centering
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_rounded_scaled_std.png}
         \caption{ }
         
     \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/2_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/2_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/2_rounded_scaled_std.png}
         \caption{}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/3_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/3_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/3_rounded_scaled_std.png}
         \caption{}
     \end{subfigure}
     \caption{We show three rounds in the maze environment. The inference and environment design is done using \texttt{ED-BIRL}. For each round, we show the constructed maze as well as the mean and the standard deviation of the posterior. Light colours denote higher values.}
\end{figure}

==> figures/mazes/maze_exp_4/maze_figure.tex <==
\begin{figure}[H]
     \centering
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[height=0.42\textwidth]{figures/mazes/maze_exp_1/1_env.png} 
         \includegraphics[height=0.42\textwidth]{figures/mazes/maze_exp_1/1_rounded_scaled_mean.png}
         \caption{}
         
     \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[height=0.42\textwidth]{figures/mazes/maze_exp_1/2_env.png}
         \includegraphics[height=0.42\textwidth]{figures/mazes/maze_exp_1/2_rounded_scaled_mean.png}
         \caption{}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[height=0.42\textwidth]{figures/mazes/maze_exp_1/3_env.png}
         \includegraphics[height=0.42\textwidth]{figures/mazes/maze_exp_1/3_rounded_scaled_mean.png}
         \caption{}
     \end{subfigure}
     \caption{     }
\end{figure}

==> sections/algorithm_maximin_next_state.tex <==
\begin{algorithm}[H]
\caption{Maximin-Regret Environment Design for Next-State Partitions}
\label{algorithm:maximin_next_state}
\begin{algorithmic}[1]
\STATE \textbf{input\,} environments $\{ \Trans_{s'}\}_{s' \in \S}$ and belief $\beta$ 
\STATE Sample a fixed set $\{\r_1, \r_2, \dots \}$ from $\beta$. % to approximate $\E_\beta [\cdot]$. 
\FOR{$n=1, 2, \dots$}
\FOR{$s'\in\S$}
\STATE Calculate
\begin{align*}
    \trans_{s'} \in \argmax_{\trans_{s'} \in \Trans_{s'}} \sum_{s\in \neigh(s')} \Big\{ \E_\beta [ \max_{a \in A} \gamma \sum_{s''\in \S} \trans_{s'} ( s'' \mid s, a) \val_\r(s'')] - \max_{b \in A}\gamma \sum_{s'' \in \S} \trans_{s'} (s'' \mid s, b) \val_{\bar \r}(s'')\Big\}
\end{align*}
\FOR{$s\in \neigh(s')$ under $\trans_{s'}$}
\vspace{0.1cm}
\STATE Set $\val_{\r} (s) \leftarrow \r (s) + \max_{a \in A} \gamma \sum_{s''\in \S} \trans_{s'} (s'' \mid s, a) \val_\r (s'')$ for every $\r \in ...$ 
\STATE Set $\val_{\bar \r} (s) \leftarrow \bar \r(s) + \max_{b \in A} \gamma \sum_{s''\in \S} \trans_{s'} (s'' \mid s, a) \val_{\bar \r} (s'')$
\vspace{0.1cm}
\ENDFOR
\ENDFOR
\ENDFOR 
\RETURN Environment $\trans = \{ \trans_s\}_{s \in \S}$ 
\end{algorithmic}
\end{algorithm} 


==> sections/algorithm_maximin_structured_belief.tex <==
\begin{algorithm}[H]
\caption{Maximin-Regret Environment Design}
\label{algorithm:maximin}
\begin{algorithmic}[1]
\STATE \textbf{input\,} Environment set $\Trans = \{\Trans_s\}_{s \in \S}$ and belief $\beta$ 
\STATE Sample a set $\mathscr{R}$ from $\beta$ used to approximate $\E_{\beta}[\cdot]$
\FOR{$n=1, 2, \dots$}
\FOR{$s\in\S$}
% \vspace{.05cm}
% \STATE Get $\trans_s \in \argmax\limits_{\trans_s \in \Trans_s} \Big\{  \E_\beta \big[ \max\limits_{a \in \A} \sum\limits_{s' \in \S} \trans_s (s'\mid s, a) \val_\r (s')\big] - \max\limits_{b \in \A} \sum\limits_{s' \in \S} \trans_s (s'\mid s, b) \val_{\bar \r}(s')\Big\}$
\STATE \begin{align*}
    \trans_s \in \argmax\limits_{\trans_s \in \Trans_s} \Big\{  \E_\beta \big[ \max_{a \in \A} \sum_{s' \in \S} \trans_s (s'\mid s, a) \val_\r (s')\big] - \max_{b \in \A} \sum_{s' \in \S} \trans_s (s'\mid s, b) \val_{\bar \r}(s')\Big\}
\end{align*} 
\STATE Set $\val_{\r} (s) \leftarrow \max_{a \in \A} \r(s) + \gamma \sum_{s' \in \S} \trans_s (s'\mid s, a) \val_\r (s')$ for $\r \in \mathscr{R}$ 
\vspace{.1cm}
\STATE Set $\val_{\bar \r} (s) \leftarrow \max_{b \in \A} \bar \r(s) + \gamma \sum_{s' \in \S} \trans_s (s'\mid s, b) \val_{\bar \r}(s')$
\vspace{0.1cm}
\ENDFOR
\ENDFOR 
\RETURN Environment $\trans = \{ \trans_s\}_{s \in \S}$ 
\end{algorithmic}
\end{algorithm} 
Ideally, we can prove that that the algorithm converges to a maximin environment. More precisely, for the approximate belief $\bar \beta$, which is estimated by sampling from $\beta$, the algorithm converges to $\trans_*$ such that $\min_{\pi \in \Pi} \bayesregret_{\bar \beta} (\trans_*, \pi) = \max_{\trans \in \Trans} \min_{\pi\in \Pi} \bayesregret (\trans, \pi)$.  

==> sections/figures/figure_continuous_mazes_selection_unused.tex <==
\begin{figure}[H]
     \centering
         \centering
         \includegraphics[width=0.95\textwidth]{figures/continuous_experiments/Maze_env_selection.png} 
        \caption{Frequency at which each continuous maze environment was picked for expert observations. The learner was allowed to observe experts in $n=10$ different environments. $\airl$, $\gail$ and $\bc$ only observed the expert on the base environment, while $\edairl$ and $\drairl$ were able to observe the expert on any environments in the demo set. For a fair comparison, we forced multi-environment approaches to always include the base environment in their selection.\label{fig:continuous_mazes_selection}}
\end{figure}

% interesting to see that env 11, 14 and 19 were never selected : they are not appealing visually neither.
% env 3 was always selected


==> sections/figures/figure_edbirl_exp.tex <==
\begin{figure}[H]
     \centering
         \begin{subfigure}[b]{0.46\textwidth}
         \centering
        %  \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_env.png} 
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.32\textwidth]{figures/mazes/maze_exp_2/1_env.png}};
            \draw (0, 1.1) node {\tiny Constructed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.32\textwidth]{figures/mazes/maze_exp_2/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
         \includegraphics[width=0.32\textwidth]{figures/mazes/maze_exp_2/1_rounded_scaled_std.png}};
            \draw (0, 1.1) node {\tiny Standard Deviation};
        \end{tikzpicture} \\
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/2_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/2_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/2_rounded_scaled_std.png}\\
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/3_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/3_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/3_rounded_scaled_std.png}
          \caption{\texttt{ED-BIRL}: Basic}

     \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.32\textwidth]{figures/mazes/maze_exp_3/1_env.png}};
            \draw (0, 1.1) node {\tiny Constructed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.32\textwidth]{figures/mazes/maze_exp_3/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.32\textwidth]{figures/mazes/maze_exp_3/1_rounded_scaled_std.png}};
            \draw (0, 1.1) node {\tiny Standard Deviation};
        \end{tikzpicture} \\
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_3/2_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_3/2_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_3/2_rounded_scaled_std.png}\\
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_3/3_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_3/3_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_3/3_rounded_scaled_std.png}
         \caption{\texttt{ED-BIRL}: Lava Bars}
     \end{subfigure}
     \caption{\textbf{\texttt{ED-BIRL}}. For two version of the maze design environment, we display three consecutive rounds. The inference and environment design is done using \texttt{ED-BIRL}. For each round, we show the constructed maze as well as the mean and the standard deviation of the estimated posterior. The computed values are scaled to $[0,1]$ and rounded. Light colours denote higher values. }
\end{figure}












==> sections/figures/figure_fixed_env_domain_random.tex <==


\begin{figure}[H]
     \centering
         \begin{subfigure}[b]{0.46\textwidth}
         \centering
        %  \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_env.png} 
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.32\textwidth]{figures/mazes/fixed_env/1_env.png}};
            \draw (0, 1.1) node {\tiny Fixed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.32\textwidth]{figures/mazes/fixed_env/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture}
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
         \includegraphics[width=0.32\textwidth]{figures/mazes/fixed_env/1_rounded_scaled_std.png}};
            \draw (0, 1.1) node {\tiny Standard Deviation};
        \end{tikzpicture} \\
         \includegraphics[height=0.32\textwidth]{figures/mazes/fixed_env/1_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/fixed_env/2_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/fixed_env/2_rounded_scaled_std.png}\\
         \includegraphics[height=0.32\textwidth]{figures/mazes/fixed_env/1_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/fixed_env/3_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/fixed_env/3_rounded_scaled_std.png}
         
         \caption{\texttt{Fixed Demo Environment}} 
     \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.32\textwidth]{figures/mazes/domain_randomisation/1_env.png}};
            \draw (0, 1.1) node {\tiny Random Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.32\textwidth]{figures/mazes/domain_randomisation/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.32\textwidth]{figures/mazes/domain_randomisation/1_rounded_scaled_std.png}};
            \draw (0, 1.1) node {\tiny Standard Deviation};
        \end{tikzpicture} \\
         \includegraphics[height=0.32\textwidth]{figures/mazes/domain_randomisation/2_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/domain_randomisation/2_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/domain_randomisation/2_rounded_scaled_std.png}\\
         \includegraphics[height=0.32\textwidth]{figures/mazes/domain_randomisation/3_env.png} 
         \includegraphics[height=0.32\textwidth]{figures/mazes/domain_randomisation/3_rounded_scaled_mean.png}
         \includegraphics[height=0.32\textwidth]{figures/mazes/domain_randomisation/3_rounded_scaled_std.png}
         \caption{\texttt{Domain Randomisation}}
     \end{subfigure}

     \caption{\texttt{Fixed Demo Environment \& Domain Randomisation.} Fixed environment and an exemplary randomly created maze. }
\end{figure}





==> sections/figures/figure_maze_basic.tex <==

\begin{figure}[H]
     \centering
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
        %  \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_env.png} 
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_2/1_env.png}};
            \draw (0, 1.1) node {\tiny Constructed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_2/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/3_rounded_scaled_mean.png}
         \caption{\texttt{ED-BIRL}}
     \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/fixed_env/1_env.png}};
            \draw (0, 1.1) node {\tiny Fixed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/fixed_env/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/fixed_env/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/fixed_env/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/fixed_env/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/fixed_env/3_rounded_scaled_mean.png}
         \caption{\texttt{Fixed Environment}}
     \end{subfigure}
           \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/domain_randomisation/1_env.png}};
            \draw (0, 1.1) node {\tiny Random Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/domain_randomisation/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/domain_randomisation/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/domain_randomisation/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/domain_randomisation/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/domain_randomisation/3_rounded_scaled_mean.png}
         \caption{\texttt{Domain Randomisation}}
     \end{subfigure}
     
     
     \caption{......}
\end{figure}


==> sections/figures/figure_maze_experiments.tex <==



\begin{figure*}[t]

     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/fixed_env/1_env.png}};
            \draw (0, 1.3) node {\tiny Fixed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/fixed_env/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/fixed_env/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/fixed_env/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/fixed_env/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/fixed_env/3_rounded_scaled_mean.png}
         \caption{\texttt{Fixed Environment\,IRL}}
                  \label{subfig:basic_fixed}

     \end{subfigure}
           \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/domain_randomisation/1_env.png}};
            \draw (0, 1.3) node {\tiny Random Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/domain_randomisation/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/domain_randomisation/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/domain_randomisation/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/domain_randomisation/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/domain_randomisation/3_rounded_scaled_mean.png}
         \caption{\texttt{Domain Randomisation}}
                  \label{subfig:basic_dom_ran}
    \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
        %  \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_env.png} 
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_2/1_env.png}};
            \draw (0, 1.3) node {\tiny Constructed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_2/1_rounded_scaled_mean.png}};
            \draw (0, 1.3) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_2/2_env.png}};
         \end{tikzpicture}
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/2_rounded_scaled_mean.png}\\
        \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_2/2_env.png}};
         \end{tikzpicture}
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/3_rounded_scaled_mean.png}
         \caption{\texttt{ED-BIRL}}
         \label{subfig:basic_ed_birl}
     \end{subfigure}
     
     \caption{Learned rewards on the maze problem. We display three consecutive rounds, the corresponding mazes and estimated rewards. We use the same colour scale as in Figure~\ref{fig:intro}, which ranges from black (0.0) to red (0.5) to white (1.0).}

     \label{fig:maze_exp}

\end{figure*}


==> sections/figures/figure_maze_experiments_4th_round.tex <==
\begin{figure*}[t]

     \centering
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
        %  \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_env.png} 
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_2/1_env.png}};
            \draw (0, 1.1) node {\tiny Constructed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_2/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/3_rounded_scaled_mean.png}
        \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/4_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_2/4_rounded_scaled_mean.png}
         \caption{\texttt{ED-BIRL}}
         \label{subfig:ed_birl_4th_round}
     \end{subfigure}

     \caption{Figure~\ref{subfig:basic_ed_birl} with an additional 4th round. We see that the reward estimate only changes marginally. Some differences can be due to the noise in the inference of BIRL. Note that the results are also rounded to the first decimal.}
     
\end{figure*}

==> sections/figures/figure_maze_lava_bars.tex <==




\begin{figure}[H]
     \centering
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
        %  \includegraphics[height=0.32\textwidth]{figures/mazes/maze_exp_2/1_env.png} 
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {\includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_3/1_env.png}};
            \draw (0, 1.1) node {\tiny Constructed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/maze_exp_3/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_3/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_3/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_3/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/maze_exp_3/3_rounded_scaled_mean.png}
         \caption{\texttt{ED-BIRL}}
     \end{subfigure}
      \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/lava_bars/fixed_env/1_env.png}};
            \draw (0, 1.1) node {\tiny Fixed Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/lava_bars/fixed_env/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/lava_bars/fixed_env/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/lava_bars/fixed_env/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/lava_bars/fixed_env/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/lava_bars/fixed_env/3_rounded_scaled_mean.png}
         \caption{\texttt{Fixed Environment}}
     \end{subfigure}
           \hfill
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/lava_bars/domain_randomisation/1_env.png}};
            \draw (0, 1.1) node {\tiny Random Maze};
        \end{tikzpicture}
         \begin{tikzpicture}
            \draw (0, 0) node[inner sep=0] {
            \includegraphics[width=0.45\textwidth]{figures/mazes/lava_bars/domain_randomisation/1_rounded_scaled_mean.png}};
            \draw (0, 1.1) node {\tiny Estimated Rewards};
        \end{tikzpicture} \\
         \includegraphics[height=0.45\textwidth]{figures/mazes/lava_bars/domain_randomisation/2_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/lava_bars/domain_randomisation/2_rounded_scaled_mean.png}\\
         \includegraphics[height=0.45\textwidth]{figures/mazes/lava_bars/domain_randomisation/3_env.png} 
         \includegraphics[height=0.45\textwidth]{figures/mazes/lava_bars/domain_randomisation/3_rounded_scaled_mean.png}
         \caption{\texttt{Domain Randomisation}}
     \end{subfigure}
     
     
     \caption{Lava Bars}
\end{figure}


==> sections/notes.tex <==
\section{Unorganised Thoughts}

Next to adaptively designing the environments, it is also interesting to compute the complete sequence of environments given $(\S, A, \trans_{\Param}, \Param, \r, \gamma)$ a priori, i.e.\ without observing expert demonstrations in between. This is slightly different from Curriculum Learning (which is typically adaptive).  


\section{Introductory Bullets}
\begin{enumerate}
    \item Reinforcement Learning (RL), recent advances 
    \item One difficulty in RL is defining a good reward function. Prone to misspecification. In particular, defining a reward function that transfers well to similar environments is challenging. 
    \item IRL is one way of dealing with this problem. IRL is generally being used to infer the reward function of agents. In particular, we do not simply wish to learn a reward which allows us to imitate agents in the current environment, but which allows us to predict their actions in other settings.
    \item Curriculum Learning (CL) for RL was introduced to support faster learning when learning the task in one go was too difficult (self-play can also be interpreted indirectly as CL)
    \item Similarly, in IRL we see that learning a good representation of the reward function is challenging, possibly too challenging. (Analogy to complicated RL problems)
    \item This inspires us to introduce CL for IRL. Similarly to CL for RL, we wish to design environments that improve learning; in our case, reward learning. 
    \item There are several unique challenges to CL for IRL: a) it is difficult to specify the objective of our learning (which is fairly easy in CL for RL). We cannot evaluate any learned reward function during training. b) as we do not know the agent's reward function, we cannot reliably anticipate the experience (i.e.\ demonstrations) that we are going to obtain from a given environment. 
\end{enumerate} 



1. environment design given a distribution over rewards (more theoretical) 

2. environment design given reward and expert policy estimates (more practical? MaxEnt?)








% Old stuff on maximin environment design


\section{Maximin Environment Design under Reward Uncertainty} 
\subsection{Objective}
\paragraph{Given a Distribution over Rewards.}
Suppose that we have a prior belief $\xi$ over rewards. Our goal is to reduce our uncertainty encoded in the distribution $\xi$. We define the Bayesian regret of a policy $\pi$ as 
\begin{align*}
    \regret (\pi, \param, \xi) = \E_{\r \sim \xi} [ \util^*(\param, \r) - \util(\pi, \param, \r)]
    \approx \sum_{\r} \xi(\r) [\util(\pi^*_{\param, \r}, \param, \r) - \util(\pi, \param, \r)],
\end{align*} 
we define $\pi^*_{\param, \r} \in \argmax_\pi \util(\pi, \param, \r)$. 
Similarly, $\pi^*_{\param, \xi}$ denotes the policy that is optimal with respect to $\xi$, i.e.\
$\pi^*_{\param, \xi} \in \argmax_\pi \E_{\r \sim \xi} [ \util(\pi, \param, \r)]$. We suggest to perform the following optimisation:
\begin{align}\label{equation:optimisation_problem}
    \max_{\param \in \Param} \min_\pi \regret(\pi, \param, \xi).
\end{align}
This can also be written as $\max_\param \regret(\pi^*_{\param, \xi}, \param, \xi)$. Note that one of the reasons we choose to maximise regret and not minimise utility is to avoid unsolvable $\param$. 
% We could approximate \eqref{equation:optimisation_problem} by performing RL updates. This would, however, require us to repeatedly solve the MDP. 


\subsubsection{Intuition and Interpretation}
\paragraph{Intuition 1: difficult, but not too difficult $\param$.}
In CL for RL the goal is generally to design environments that are challenging for the current policy, but are still solvable for a (slightly) better policy. By maximising the Bayesian regret, we design environments $\param$ that are difficult to solve for the currently best (myopic/stationary) policy $\pi^*_{\param, \xi}$ w.r.t.\ our belief. However, we also choose $\param$ to be easy to solve (rewarding) under every single reward $\r$ with policy $\pi^*_{\param, \r}$. 

\begin{example}[Intuition 2]
Consider the belief with $\xi(\r_1) = \xi(\r_2) = \frac{1}{2}$. For any environment $\param$, there are optimal policies $\pi^*_{\param, \r_1}$ and $\pi^*_{\param, \r_2}$. W.l.o.g.\ let us assume that $\r_1$ is the true reward function. Suppose that we choose $\param$ such that $\pi^*_{\param, \r_1} = \pi^*_{\param, \r_2}$ (or their trajectories are equal for MaxEnt stuff, whatever). Well, for this choice of $\param$, we have $\regret(\pi^*_{\param, \xi}, \param, \xi) = 0$, since $\pi^*_{\param, \xi}$ maximises utility under both $\r_1$ and $\r_2$. Analogously, if we choose $\param$ such that $\regret(\pi^*_{\param, \xi}, \param, \xi) = 0$, we can expect to have $\pi^*_{\param, \r_1} \approx \pi^*_{\param, \r_2}$. Is this choice of $\param$ good? No! When we observe $\pi^*_{\param, \r_1}$ (as $\r_1$ is w.l.o.g.\ assumed to be the true reward function), we get no information at all about whether $\r_1$ or $\r_2$ is the true reward function. The reward function are equivalent under such $\param$.  

Now, suppose we choose $\param$ such that $\regret(\pi^*_{\param, \xi}, \param, \xi) > 0$. This implies that $\pi^*_{\param, \r_1} \neq \pi^*_{\param, \r_2}$. To see this, assume the contrary. Then, $\pi^*_{\param, \xi} = \pi^*_{\param, \r_1} = \pi^*_{\param, \r_2}$ and the regret has to be zero. Now, when we observe the expert in $\param$, we will observe (w.l.o.g.) $\pi^*_{\param, \r_1} \neq \pi^*_{\param, \r_2}$, ruling out the alternative $\r_2$.  
\end{example}


\paragraph{Interpretation:} Can we relate equation~\eqref{equation:optimisation_problem} to a notion of information gain?

% \begin{align*}
%     \max_\param \min_\pi \E_{\r \sim \xi} \left[ \util^*(\param, \r) \right] - \E_{\r \sim \xi} \left[ \util (\pi, \param, \r))\right] \\
%     \max_\param \E_{\r \sim \xi} \left[ \util^*(\param, \r) \right] - \E_{\r \sim \xi} \left[ \util(\pi^*_{\param, \xi}, \param, \r) \right].  
% \end{align*}
% One problem is that there is, to my knowledge, no computationally efficient way to estimate a posterior $\xi_t$. 

\subsection{Given Candidate Rewards}
Most non-Bayesian IRL algorithms do not approximate a distribution over reward functions, but instead provide a single candidate reward (e.g.\ MaxEntIRL). Let $\r_1, \dots, \r_t$ be the candidate reward functions obtained form running IRL with demonstrations $\tau_1, \dots, \tau_t$ in environments $\param_1, \dots, \param_t$, respectively.\footnote{One could also consider $\r_1, \dots, \r_t$ that are being computed by running Multi-Environment IRL for all past observations every round.} One possibly reasonable way to reduce our ambiguity about the reward function is to solve for the following:
\begin{align}
    \max_\param \min_\pi \E_{\r \sim \mathcal{U}(\r_1, \dots, \r_t)} \left[ \util^*(\param, \r) \right] - \E_{\r \sim \mathcal{U}(\r_1, \dots, \r_t)} \left[ \util(\pi, \param, \r) \right].
\end{align}

\paragraph{Something computationally efficient?} For something computationally efficient, it may make sense to do something like  
\begin{align}
    \argmax_{\param \in \Param} \sum_{i=1}^t \util(\tau_i, \param, \r_i) - \util(\tau_i, \param, \xi), 
\end{align}
or, 
\begin{align}
    \argmax_{\param \in \Param} \sum_{i=1}^t \util(\hat \pi_i, \param, \r_i) - \util(\hat \pi_i, \param, \hat \r),
\end{align}
where $\hat \r$ is the result of ME-IRL. 
One can also swap $\tau_i$ by an estimated expert policy $\hat \pi_i$ when available. 
Arguably, this can be done in an efficient way for any problem instance, as we only need to evaluate the trajectories $\tau_i$ in each environment $(\param, \r_i)$. This in fact also prevents us from choosing environments $\param$ such that any trajectory completely fails, since otherwise the difference in utility is zero. 


\subsection{Ideas?!}
Try a Dual-MDP formulation as in \cite{zhang2017learning}.

Try something like in \cite{ramponi2021learning}. 


Would it make sense to optimise for $\tilde \r \defn \sum_{i=1}^m \lvert \hat \r_i - \hat \r_{1:m} \rvert$? 

If we have $\tilde \r \defn \sum_{i=1}^m (\hat \r_i - \hat \r_{1:m})^2$ and $\hat \r_{1:m} = \frac{1}{m} \sum_{i} \hat \r_i$, we could interpret $\r$ as a sample variance? 

So, for a distribution $\beta$ over rewards: $\tilde \r \defn \E_{\r \sim \beta} [ (\r - \bar \r)^2]$ with $\bar \r$ being the mean of $\beta$. 

Trying to make the expert visit states with high variance? 

We could design a Dual MDP with rewards $\tilde \r$? 

Maybe, $\max_\param \util( \pi(\hat \r_{1:m}, \param), \tilde \r, \param)$? 


$\pi(\hat \r_{1:m}, \param)$ is our best guess of the behaviour of the expert in environment $\param$. 

Arguably, the more states the expert visits (is allowed to visit), where $\hat \r_{1:m}$ and $\hat \r_i$ disagree, the more ... 

==> sections/notes_2.tex <==


\section{Motivational Examples} 

\begin{itemize}
    \item IRL for autonomous driving. Human driving demonstrations from what city in the US are most informative and what is the best combination of test driving locations in order to learn about a human driver's reward function (their high-level intentions while driving). 
    
    The space of environments could be e.g.\ different cities, or rural areas / downtown / highway. 
    
    \item Learning user preferences in a social networks. What slightly different user interface should I provide a (test) user with in order to learn their preferences correctly? 
    
    The space of environments could be seen as a set of slightly different user interfaces or interface dynamics. 
    
    \item Essentially any problem for which it is difficult to specify a reward function and we are able to let a human play e.g.\ slightly different versions of a game (with slightly different rules).
\end{itemize}


\section{Notes: Experiments}
\subsection{Domains}
\begin{enumerate}
    \item \textbf{Maze Environment}
    
    Method: \textbf{Brute-Force + Bayesian IRL}
    
    Purpose: Illustrating the ED process (early on in the paper) and show that we can recover the reward function by adaptive environment design
    
    \item \textbf{Stochastic Shortest Path} \\ 
    with a) finite structured environment set, b) continuous perturbations
    
    Method: \textbf{Extended VI + Bayesian IRL} 
    
    Purpose: A problem for which we can use Extended VI. Show that we can recover the reward function as well as sample-efficiency and robustness. 
    
    \item \textbf{Standard Complex, Continuous Control Benchmarks} such as Ant \\ with small, finite environment set (see e.g.\ \cite{fu2017learning, chae2022robust}) 
    
    Method: \textbf{Brute Force + Adversarial IRL}
    
    Purpose: Show the sample-efficiency and robustness of learnt rewards with the goal of demonstrating performance improvements.
    
\end{enumerate}


\subsection{Experimental Setup }
Experimental setups for the above domains: 

\begin{enumerate}
    \item Experiment~1: Have a set of demo environments $\Trans_{demo}$ and a set of test environments $\Trans_{test}$. Compare a) performance in a single demo environment, b) repeatedly choosing random demo environment, c) \texttt{ED-AIRL}. Consider average performance across all test environments 
    \item Experiment~2 (Special Case of Experiment~1): Several demo environments $\Trans_{demo}$ which possibly are all different from the \emph{single} test environment $\Trans_{test}=\{\trans_{test}\}$. Compare versus observing expert in (only) the test environment. In this case, we can also compare against Imitation Learning. 
    \item Experiment~3 (Special Case of Experiment~1/2): Assume that only the \emph{initial state distribution} can be varied in the demo environments. 
\end{enumerate}
Move the (set of) target MDPs further and further away from $\Trans$. Start of with MDPs inside the convex hull and move further away (like Hannes does in his Transfer RL work). 

\paragraph{Special Case: Initial State Distributions}
Consider the special case when we can select the initial state distribution of the demonstrating expert, but cannot vary anything else in the environment. This most likely does not make a huge difference, but should (slightly) increase sample-efficiency. 

Note that this \textbf{can be done efficiently}, since we need to compute the optimal policies w.r.t.\ different rewards only for one environment. The rest can then be evaluated using rollouts.  




\subsection{Preliminary Results}


Posterior Mean for Regret-Based Adaptive Environment Design. By adaptively designing environments, we can recover the true reward function. Clearly, from observations in a single environment, it is impossible to recover the complete reward function (since only the closest reward state is being visited by the expert). Moreover, domain randomisation can produce entirely unsolvable environments and can fail to explore the reward function in detail. Optional (e)-(h): sequence of environments leading to these posteriors. [Placeholders]

% \section{...}

% CLAIM: In particular, note that for Maximum-Entropy IRL as well as Bayesian IRL $\hat \r_{1:m} = \hat \r_i$ if $\hat \r_1 = \dots = \hat \r_m$. In other words, there is no uncertainty. 

% This is similar to saying $\r_1 = \dots = \r_m$ with $\r_1, \dots, \r_m \sim \beta$. 




















\section{Environment Design for IRL} 

We consider two different scenarios. Firstly, the case when we can retrieve a (Bayesian) belief $\beta (\cdot \mid \data_{1:k})$ about the reward function in round $k$, e.g.\ by means of sampling-based Bayesian IRL. Secondly, the case when we obtain a single estimate of the reward functions based on our observations only, e.g.\ by means of Max-Ent IRL. 
Having a Bayesian belief about the reward function has the advantage that it gives us a principled way to reason under and about uncertainty. This is key as one main goal of the environment design process is to reduce the uncertainty about the reward function.\footnote{Note that another goal could be to design environments that prevent the overfitting of reward learning to specific environment dynamics.} We will initially explain how to generate environments in this case and then later explain what to do deal with point estimates (as in Max-Ent IRL). 

Moreover, the structure of the environment set $\Trans$ is crucial. In a first step, we consider the case when $\Trans$ is continuous and transitions "independent". Then, we consider the less benign case where $\Trans$ is discontinuous and exhibits no useful structure (and we actually do not explicitly know $\Trans$, but only have access to corresponding simulators). 

It is also interesting to only consider the initial state and find the most informative starting position. This can for instance be done by fixing all transitions $\trans_s$ except for $\trans_{s_0}$, where $s_0$ is a dummy state. 
Interestingly, we do not have to adapt IRL methods in this case as transitions remain the same. 

Moreover, it is also interesting to analyse the environment design process for the completely oblivious belief, i.e.\ a uniform prior over reward functions. What is the best environment to learn from when we have no clue about the rewards whatsoever? 

\subsection{Environment Generation via Maximin Bayesian Regret} 

\textbf{A similar idea was used in "Risk-Aware Active Inverse Reinforcement Learning". It's a performance related objective (not only uncertainty related objective). \cite{brown2018efficient, brown2018risk}} 

Let $\val(\trans, \r, \pi)$ denote the value function and $\omega$ the initial state distribution.
We define the Bayesian regret of an environment $\trans$ and policy $\pi$ under belief $\beta$ as 
\begin{align}
    \bayesregret_\beta (\trans, \pi) \coloneqq \E_{\r \sim \beta} \big[\max_{\pi'} \mathcal{V}(\trans, \r, \pi', \omega) - \mathcal{V}(\trans, \r, \pi, \omega) \big]    
\end{align}
We could also consider the initial state distribution as part of the environment and introduce an initial state $s_0$ whose transitions $\trans_{s_0}$ we can modify.
We propose the following maximin regret objective for our environment design process:  
\begin{align*}
    \max_{\trans \in \Trans} \min_{\pi\in \Pi} \bayesregret_\beta (\trans, \pi). 
\end{align*}
What this means is that we search for an environment such that an agent maximising for specific $\r$ sampled from the belief $\beta$ performs maximally better than an agent assuming that the mean $\bar \r = \E_{\r \sim \beta} [\r]$ is an accurate representation of the reward function. 

This is equivalent to: 
\begin{align*}
    \max_{\trans} \big\{ \E_{\r \sim \beta} [\max_{\pi'} \mathcal{V}(\trans, \r, \pi', \omega)] - \max_{\pi} \E_{\r \sim \beta}[\mathcal{V}(\trans, \r, \pi, \omega)] \big\}. 
\end{align*}
Again, we can simplify by noting that $\E_{\r \sim \beta}[\mathcal{V}(\trans, \r, \pi, \omega)] = \mathcal{V}(\trans, \bar \r, \pi, \omega)$ with $\bar \r = \E_{\r \sim \beta} [\r]$.  
Maximising the regret objective also has the advantage that the expert should typically be able to solve the environments (as the regret in degenerate or purely adversarial environments will typically be close to zero). Moreover, note that if the objective becomes zero and in a Bayesian setup the prior included the actual reward function, then we are guaranteed to perform optimally in every environment in $\Trans$ (under any reward function from the belief and in particular $\bar \r$. 

If we want to do something for the state-occupancy instead of the utility, we could consider something like 
\begin{align*}
    \argmax_{\trans \in \Trans} \lVert \E_{\r \sim \beta} [\varphi (\pi_{\r, \trans}, \trans)] - \varphi(\pi_{\bar \r, \trans}, \trans)]\rVert
\end{align*}
where $\pi_{\r, \trans}$ is the optimal policy w.r.t.\ $\r$ and $\trans$,  $\varphi(\pi, \trans)$ is the state-occupancy of policy $\pi$ in environment $\trans$, and $\lVert \cdot \rVert$ an appropriate norm. However, I don't see how to optimise this efficiently. 

\paragraph{Structured Environment Configurations.} Let $\trans_s \in \Reals^{\S \times A}$ denote a transition matrix dictating the transition probabilities in state $s$. Clearly, we can identify any transition function $\trans$ with a family of state transition matrices $\{\trans_s\}_{s\in \S}$. We now say that an environment set $\Trans$ allows us to make independent transition choices if there exist sets of transition matrices $\Trans_s$ for $s \in \S$ such that $\Trans = \{ \{ \trans_s\}_{s \in \S} \colon \trans_s \in \Trans_s\}$.   

Essentially, what this means is that we can combine any environment changes in a state $s$ with any changes in another state $s'$. This should allow us to optimise somewhat efficiently, e.g., by means of dynamic programming. 

\input{sections/algorithm_maximin_structured_belief}
% \begin{align*}
%     & V^\trans (s) = \max_{\trans_s \in \Trans_s} \Big\{ \E_\beta [ \max_{a \in \A} \r(s) + \gamma \sum_{s'} \trans_s ( s' \mid s, a) V^\r(s')] - \max_{b \in \A} \bar \r(s) + \gamma \sum_{s'} \trans_s (s' \mid s, b) V^{\bar \r}(s') \Big\} \\
%     & V^\r (s) = \max_{a \in \A} \r(s) + \gamma \sum_{s'} \trans_s (s' \mid s, a) V^\r (s') \qquad [\textit{for every } \r \textit{ from } \beta] \\ 
%     & V^{\bar \r} (s) = \max_{b \in \A} \bar \r(s) + \gamma \sum_{s'} \trans_s (s' \mid s, a) V^{\bar \r} (s')
% \end{align*}

Can this give you cycles? I don't think so. 

The computed value functions should be "aligned", since it's max-max and max-min. 


How to deal with continuous $\Trans_s$? How to deal with continuous state/action spaces? 

Note that we consider discounted infinite horizon MDPs. %The time dependence in Backwards Induction could otherwise mess things up (and we can only get something approximate by, e.g., fixing $\trans_s$ the first time state $s$ is considered)

I guess, one can write it more concisely by defining Bellman optimality operators w.r.t.\ $\r$ and $\trans_s$. 

See also Algorithm~\ref{algorithm:maximin_next_state} in the Appendix for a slightly different case. 


\subsection{Unstructured Environment Configurations} 
Let's consider the situation when the environment set $\Trans$ has no useful structure. Moreover, suppose that we don't know the transition functions in $\Trans$ explicitly, but are only able to access corresponding simulators. This is as general as we can make the environment design setting and such situations may reasonably occur in practice quite often. In this case, we cannot hope to solve any optimisation problem over the environments particularly efficiently or precisely. In particular, lacking structure in the environment set, we can only approximate the maximin-regret objective of Section~X by choosing a random subset $\Trans_\subseteq \subseteq \Trans$ and compute $\max_{\trans\in \Trans_\subseteq} \min_{\pi \in \Pi} \bayesregret_\beta (\trans, \pi)$. However, this requires us to solve MDPs in an inner-loop. More specifically, we would need to solve $|\Trans_\subseteq| \times (|\beta| + 1)$ many MDPs, where $|\beta|$ denotes the sample size taken from the belief. This appears to be very impractical. 

Alternatively, one idea is not to compare the behaviour implied by reward functions (as the Bayesian regret does), but to compare reward functions directly. Since $\bar \r$ is the best estimate of the reward function available, we estimate the expert's behaviour by calculating $\pi_{\bar \r, \trans} \in \argmax_\pi \util(\pi, \trans, \bar \r)$ for every $\trans \in \Trans_\subseteq$. We then choose the environment (in $\Trans_\subseteq$) in which the belief disagrees the most with the mean under the state-occupancy generated by policies $\pi_{\bar \r, \trans}$ in environments $\trans \in \Trans_\subseteq$, i.e.\ 
\begin{align*}
    \argmax_{\trans \in \Trans_\subseteq} \E_{\r \sim \beta} \Big[ \big\lvert \util(\pi_{\bar \r, \trans}, \trans, \bar \r) - \util(\pi_{\bar \r, \trans}, \trans, \r) \big\rvert \Big].
\end{align*} 
Note that taking absolute values is important as the above would otherwise be zero always. This approach requires solving "only" $|\Trans_\subseteq|$-many MDPs as well as performing roll-outs to estimate the utility. In particular, it only requires access to simulators in order to train policies $\pi_{\bar \r, \trans}$. This might be especially useful in domains with large/continuous state and action spaces. 

\paragraph{Maximising Variance under Expected State-Occupancy.} A slightly different version of this would be to maximise the \emph{outcome variance of $\beta$ under the expected policy $\pi_{\bar \r, \trans}$}. More precisely, we want to maximise $\E_{\beta} [ \varphi(\pi_{\bar \r, \trans})^\top (\r- \bar \r)^2]$, that is, the square difference in rewards under the state-occupancy $\varphi(\pi_{\bar \r, \trans})$. We can write equivalently 
\begin{align}
    \argmax_{\trans \in \Trans_\subseteq} \E_{\r \sim \beta, s \sim \varphi(\pi_{\bar \r, \trans})} \big[ \big(\r(s) - \bar \r(s)\big)^2 \big]. 
\end{align}
One can interpret the above also as a variance of the belief under the expected state-occupancy in a given environment: $\max\limits_{\trans} \var_{\varphi(\pi_{\bar \r, \trans})}(\beta)$. 

Algorithm: Compute $\pi_{\bar \r, \trans}$ for all $\trans \in \Trans_\subseteq$. Then take the argmax over $\trans$ of the expression above. 

This should create environments in which the expert tends to visit states, where the standard deviation, i.e.\ variance, of $\beta$ is large.  

Variance-Induced Environment Design (\textsc{VarIED}). The idea is quite simple. Choose an environment such that the expert visits regions of the state space about whose rewards we are uncertain (high variance). Clearly, we cannot accurately predict the expert's behaviour as we do not know their reward function. Thus, we instead use the estimated state-occupancy under $\pi_{\bar \r, \trans}$, i.e.\ our currently best prediction of the expert's behaviour. 



\textbf{Note that any (easy to compute) concept can be used instead of the variance of $\beta$. For instance, some kind of information gain / entropy. See the Active Learning in IRL literature for some choices / objectives.}

% In the above, it may more make more sense to compare the \emph{occupancy measures} induces by the reward functions instead of the utility. We essentially use the utility as a proxy for the occupancy measure. 


% \subsection{Optimistic Environment Design}
% Another idea that could be applied to structured environment sets could be to search in the space of optimistic environments. 
% \begin{enumerate}
%     \item Sample $\r_1, \dots, \r_m$ from $\bel$.
%     \item Compute $(\param_i, \pi_i) \in \argmax_{\param, \pi} \util(\pi, \param, \r_i)$; the optimistic environments for rewards $\r_i$  
%     \item Compute $\param^* \in \argmax_{\param_i, \pi_i} \sum_{j \neq i} \big\lvert \util(\pi_i, \param_i, \r_i) -  \util(\pi_i, \param_i, \r_j)\big\rvert $; 
% \end{enumerate}
% % Notation: It's nicer to write $\r_i(\pi_i, \param_i) - \r_j (\pi_i, \param_i)$. 
% Step 2) can be calculated by extended value iteration for environment sets with independent transition changes. Step 3) requires policy roll-outs, but is otherwise computationally efficient. 



\subsection{Environment Design with Point Estimates}
So far we assumed access to a belief distribution over rewards, e.g.\ a prior or posterior over reward functions, which is typically available when the learner takes a Bayesian perspective and aims to estimate a posterior over reward functions. This has the advantage that we have a principled way to reason about our uncertainty. However, many popular IRL methods, such as Maximum-Entropy IRL, compute only point estimates, i.e.\ they compute a single best guess about the reward function based on available observations. In this case, it is not clear on what to base the design of demo environments on. 

Having no principled way to reason about our uncertainty, we propose the following assumption and intuition. 


\begin{assumption}
     If $\algo(\data_{1:k})$ is my current best guess about the reward function and $\algo(\data_i)$ is widely different from $\algo(\data_{1:k})$, then an expert demonstration that distinguishes $\algo(\data_{1:k})$ from $\algo(\data_i)$ improves my estimate about the reward function in round $k+1$, i.e.\ $\algo(\data_{1:k+1})$. 
\end{assumption} 


\begin{remark}
For MaxEnt IRL, if $\r_1 = \dots = \r_m$, then $\r_{1:m} = \r_1$. 
\end{remark}

(Before: Environment Design with Bayesian Beliefs)

To resolve this issue, we introduce a pseudo-belief over reward functions. The pseudo-belief is given by $\hat \beta = \mathcal{U}(\r_{\data_1}, \dots, \r_{\data_m})$ and $\r_{\data} \approx \E[\hat \beta]$. 


Bayesian IRL methods correspond to a function $G: \mathscr{D} \to \mathscr{B}$, whereas, e.g., MaxEnt IRL corresponds to a function $G: \mathscr{D} \to \mathscr{R}$. 

We artificially generate a belief about the reward function by making the following assumption: Our current best guess $\r_{1:m} = \algo(\data_1, \dots, \data_m)$ based on all available data $\data_1, \dots, \data_m$ is constructed from $\r_1 = \algo(\data_1), \dots, \r_m = \algo(\data_m)$. 

Note that it makes some sense to consider $\mathcal{U}(\r_1, \dots, \r_m)$ as the pseudo-belief, as (for MaxEnt IRL) if $\r_1 = \dots = \r_m$, it follows that $\r_{1:m} = \r_1$. 


---------

\section{12.09}






For notation, see Section~2. 

\begin{algorithm}[H]
\caption{Environment Design with Beliefs}
\begin{algorithmic}[1]
\STATE \textbf{input\,} set of environments $\Trans$, resources $m \in \mathbb{N}$, prior $\P(\cdot)$ 
\FOR{$k = 1, \dots, m$}
\STATE Sample rewards from $\P(\cdot \mid \data_{1:{k-1}})$ and construct empirical distribution $\hat \P_{k-1}$
\STATE Derive best guess $\bestR$ from $\hat \P_{k-1}$, e.g.\ posterior mean or MAP reward
\vspace{.05cm}
\STATE Choose the demo environment in an either regret- or uncertainty-based fashion:
\[
    \trans \in \begin{cases}
        \argmax\limits_{\trans \in \Trans} \bayesregret_{\hat \P_{k-1}}(\pi^*_{\bestR, \trans}, \trans), & \text{(Section~\ref{subsection:max_regret_ed})}
		\\[1em]
		\argmax\limits_{\trans\in \Trans} \varphi(\pi^*_{\bestR, \trans}, \trans)^\top H(\hat \P_{k-1} \mid \trans), & \text{(Section~\ref{subsection:max_entropy_ed})}
		
		\end{cases}
\]
\STATE Observe expert trajectory $\tau_{k}$ in environment $\trans_{k}$  
\ENDFOR
\STATE Final run of IRL for all observations $\data_{1:m}$
\end{algorithmic}
\end{algorithm} 


\begin{algorithm}[H]
\caption{Environment Design with Point Estimates}
\begin{algorithmic}[1]
\STATE \textbf{input\,} set of environments $\Trans$, resources $m \in \mathbb{N}$ 
\STATE For $k = 1, 2$ simply let $\hat \P_{k-1}$ equal, for instance, an empirical uniform distribution  
\FOR{$k = 3, \dots, m$}
\STATE Get point estimates $\r_i = \mathcal{G}(\data_i)$ for $i < k$ and let $\hat \P_{k-1} \equiv \mathcal{U}(\r_1, \dots, \r_k)$
\STATE Derive best guess $\bestR = \mathcal{G}(\data_{1:{k-1}})$ using all past observations
\vspace{.05cm}
\STATE Choose the demo environment in an either regret- or uncertainty-based fashion:
\[
    \trans \in \begin{cases}
        \argmax\limits_{\trans \in \Trans} \bayesregret_{\hat \P_{k-1}}(\pi^*_{\bestR, \trans}, \trans), & \text{(Section~\ref{subsection:max_regret_ed})}
		\\[1em]
		\argmax\limits_{\trans\in \Trans} \varphi(\pi^*_{\bestR, \trans}, \trans)^\top H(\hat \P_{k-1} \mid \trans), & \text{(Section~\ref{subsection:max_entropy_ed})}
		
		\end{cases}
\]
\STATE Observe expert trajectory $\tau_{k}$ in environment $\trans_{k}$  
\ENDFOR
\STATE Final run of IRL for all observations $\data_{1:m}$
% \STATE (Here, $\mathcal{G}$ denotes a generic IRL algorithm that computes point estimates of the reward function.) 
\end{algorithmic}
\end{algorithm} 



We refer to the combination of Environment Design with Beliefs (Algorithm~3) with Bayesian IRL (Section~2) as \texttt{ED-BIRL}. Similarly, we denote by \texttt{ED-AIRL} the combination of Environment Design with Point Estimates (Algorithm~4) with Adversarial IRL (Algorithm~2).  




\subsection{Minimax Bayesian Regret Environment Design} \label{subsection:max_regret_ed} 
Choose environment $\trans$ such that the optimal policy with respect to the learner's best guess $\bestR$ suffers maximal (Bayesian) regret under the distribution $\P(\r \mid \data)$ in $\trans$. \textbf{General description of the objective etc.}


\paragraph{Structured Environments.} Often the environment set has a useful structure that we can exploit in order to search the space of environments efficiently. 



\paragraph{Arbitrary Environments.} In some situations, the set of demo environments $\Trans$ may not exhibit any useful structure. Moreover, we may not even have explicit knowledge of the transition functions in $\Trans$, but can only access a set of corresponding simulators $\mathscr{S}$. In this case, we are left with approximating the minimax regret objective (...) by sampling simulators and performing rollouts, see Algorithm~\ref{algorithm:brute_force_ed}.






\begin{algorithm}[H]
\caption{Continuous Perturbations}
\begin{algorithmic}[1]
\STATE \textbf{input} $\{\varepsilon_{s,a}\}_{s, a}$
\STATE \textbf{repeat} until $\val_{\bestR}$ and $\val_{\r}$ for $\r \in \mathcal{R}$ converge: 
\FOR{$s\in\S$}
\FOR{$a \in \A$}
\STATE $\Delta_{s,a} \leftarrow \argmax\limits_{\mathbf{1}^\top\Delta=0, \lVert \Delta \rVert_2 \leq \varepsilon_{s,a}} (\trans_{s,a} + \Delta )^\top (\E_\r [\val_\r] - \val_{\bar \r} )$ 
\STATE This is just $\Delta_{s,a}(s_{\max}) = \varepsilon /2$ and $\Delta(s, a) (s_{\min}) = \varepsilon/2$ with $s_{\max} = \max_s (\E_\r [\val_\r(s)] - \val_{\bar \r}(s))$ and $s_{\min} = \min_s (\E_\r [\val_\r(s)] - \val_{\bar \r}(s))$
\ENDFOR
\STATE $\val_{\r} (s) \leftarrow \max\limits_{a \in \A} \r(s) + \gamma  \big(\trans_{s, a} + \Delta_{s,a}\big)^\top \val_\r$ \qquad for $\r \in \mathcal{R}$
\STATE $\val_{\bar \r} (s) \leftarrow \max\limits_{b \in \A} \bar \r(s) + \gamma \big(\trans_{s, b} + \Delta_{s,b}\big)^\top \val_{\bar \r}$
\ENDFOR 
\RETURN Environment $\trans^\Delta = \{\trans^\Delta_{s,a}\}_{s,a}$ with $\trans^\Delta_{s,a} \defn \trans_{s, a} + \Delta_{s,a}$
\end{algorithmic}
\end{algorithm} 


Note: In addition to unstructured finite many environments and structured finite many environments (according to states), we may also look at \textbf{continuous perturbations of a base MDP}. If these perturbation are made for each state-action pair separately, e.g.\ we have some sort of $L_2$-$\varepsilon$-ball around the transitions for each state, then the Extended VI approach should still work (to find the argmax we likely have to use gradient ascent, which is fine, since the objective is linear in the transition changes). Roughly speaking, in Extended VI we then optimise: (Maybe not as obvious how to do it)
\begin{equation}
    \Delta_{s,a} = \argmax_{\lVert \Delta\rVert_1 = 0, \lVert \Delta \rVert_2 \leq \varepsilon} \E_\r \max_a (\trans_{s, a} + \Delta)^\top \val_{\r} - \max_b (\trans_{s, b} + \Delta)^\top \val_{\bestR} 
\end{equation} 









\subsection{Maximal State Entropy Environment Design}\label{subsection:max_entropy_ed}
Choose environment $\trans$ such that we can expect to observe the expert in states with large uncertainty (entropy) about the optimal action under $\P(\r \mid \data)$. 

% Choose environment $\trans$ such that a policy maximising for rewards sampled from $\P(\r \mid \data)$ and $\trans$ exhibits maximal entropy. 

See \url{https://flowers.inria.fr/mlopes/myrefs/09-ecml-airl.pdf} for $H$ 
































\section{Maximin Environment Design for Maze Environments} 

When we want to generate mazes by placing walls on tiles in a gridworld, the environment configurations do not partition as considered in Section~X for a standard state encoding. Therefore, instead of starting state independent transition changes as considered in Section~X, we now consider next state independent transition changes. To this end, let $\trans_{s'}$ denote the transition matrices dictating the transitions \emph{to} state $s'$ and define $\Trans_{s'}$ accordingly. Let $\neigh(s')$ denote the states from which state $s'$ is reachable under some $\trans_{s'} \in \Trans_{s'}$. Thus, in the example of mazes $\neigh(s')$ denotes the neighbouring tiles of tile $s'$. In that case, the collection $\Trans_{s'}$ consists only of two matrices, the zero-matrix, under which $s'$ is a blocked state, and the matrix where $s'$ can be visited from its neighbouring states. The Extended Value Iteration for this case is slightly more involved, but essentially the same: 

\input{sections/algorithm_maximin_next_state}


I feel like this can give you cycles. Not sure though. 

Note that $\trans_{s'}(s'' \mid s, a)$ is not influenced by $\trans_{s'}$ apart from the case when $s'' = s'$. 

Looks a bit like Asynchronous Dynamics Programming as we update some states more frequently than others (the MDP should be connected for this to work). 

For mazes, we can also view $\trans_{s'}$ as a parameter $\param_{s'}$ with two values so that $s'$ is blocked when $\param_{s'} = 1$ and free if $\param_{s'} = 0$. That's how one would code this anyways. 



% Algorithms may actually be capable of saying, "no more additional demonstrations needed" as it does not expect any information gain. 





\section{Reasons for Overfitting in IRL} 
\emph{Why do certain IRL methods overfit to the demo environment?} [Even in "Robust IRL" \cite{fu2017learning} one can see in their experiments that their method overfits to the trajectory / state-visitations of the trajectory.] A high-level reason can be that with the original goal of imitation learning you test on your training environment. Thus, overfitting is good / not harmful. 

I don't think IRL directly overfits to environments dynamics, but that it overfits to the state-visitation frequencies of observed trajectories. And, as the state-visitation frequencies heavily depend on the environment dynamics (next to the reward function), this in turn makes IRL overfit rewards to the transition function. \emph{Why does IRL overfit to state-visitation frequencies?}



% I think this is due to the trajectory being generated by a specific environment. States along the trajectory path will always have higher rewards (the likelihood is larger under such rewards). Note that Max-Ent IRL as well as Bayesian IRL consider the likelihood (and maximise or perform weighting w.r.t.\ it). 


It's seems like IRL methods are actually estimating the value of a state, which is dynamics dependent, and not the reward function. 


\vspace{1cm}

$\tau$ is generated by the environment dynamics $\trans$ and some (unknown) optimal policy $\pi$. 
\begin{align*}
    p(\tau \mid \r) = \prod_{(s,a) \in \tau} \frac{e^{\alpha Q^\r(s, a)}}{\sum_{a'} e^{\alpha Q^\r(s,a')}}
\end{align*}
Maximising this begs you to overfit to the dynamics underlying $Q$ and the generation of $\tau$, doesn't it? 
It seems that you want to fit a Q-function along the trajectory path (and only along this path). 


% \subsection{... and Preventive Measures} 



\subsection{...}

From Lopes et al:

It is worth mentioning that, in the context of IRL, there are two main sources
of uncertainty in recovering the reward function. One depends on the natural
ambiguity of the problem: for any particular policy, there are typically multiple
reward functions that solve the IRL problem. This type of ambiguity appear
even with perfect knowledge of the policy, and is therefore independent of the
particular process by which states are sampled. The other source of uncertainty
arises from the fact that the policy is not accurately specified in certain states.
This class of ambiguity can be addressed by sampling these states until the policy
is properly specified. Our entropy-based criterion does precisely this.





\begin{algorithm}[H]
\caption{Continuous Perturbations: Gradients?}
\begin{algorithmic}[1]
\STATE \textbf{input} base transitions $\trans$, radii $\{\varepsilon_{s,a}\}_{s, a}$
\STATE Pre-train value functions and policies on base environment
\STATE \textbf{repeat} 
\FOR{$s\in\S$}
\FOR{$a \in \A$}
\STATE $\Delta_{s,a} \leftarrow \mathrm{Proj}_{\varepsilon_{s, a}} \big( \Delta_{s, a} + \eta \nabla G_{\val, \pi}(\Delta_{s, a})\big)$ 
\ENDFOR
\STATE $\val_{\r} (s) \leftarrow \max\limits_{a \in \A} \r(s) + \gamma  \big(\trans_{s, a} + \Delta_{s,a}\big)^\top \val_\r$ \qquad for $\r \in \mathcal{R}$
\STATE $\val_{\bar \r} (s) \leftarrow \max\limits_{b \in \A} \bar \r(s) + \gamma \big(\trans_{s, b} + \Delta_{s,b}\big)^\top \val_{\bar \r}$
\STATE $\pi_\r \leftarrow ...$
\STATE $\pi_{\bar \r} \leftarrow ...$
\ENDFOR 
\RETURN Environment $\trans^\Delta = \{\trans^\Delta_{s,a}\}_{s,a}$ with $\trans^\Delta_{s,a} \defn \trans_{s, a} + \Delta_{s,a}$
\end{algorithmic}
\end{algorithm} 

Define $g: \Reals^{|\S|} \to \Reals$ as $$g(\Delta_{s,a}) = \E_{\r} \left[ \ind_{\{ \pi^R(s) = a\}} (\trans_{s, a} + \Delta_{s, a})^\top \val_\r \right] - \ind_{\{ \pi^{\bar \r} = a\}} (\trans_{s, a} + \Delta_{s, a})^\top \val_{\bar \r}$$

$$ \frac{\partial g(\Delta_{s, a})}{\partial \Delta_{s, a, s'}} = \E_{\r} \left[ \ind_{\{ \pi^R(s) = a\}} (\trans_{s, a} + \mathbf{e}_{s'})^\top \val_\r \right] - \ind_{\{ \pi^{\bar \r} = a\}} (\trans_{s, a} +  \mathbf{e}_{s'})^\top \val_{\bar \r} $$ 


I guess for any (continuous) parameter space $\Theta$ we could optimise any objective by doing gradient ascent, where for each gradient step we find the optimal policies.  


==> sections/proof_notes.tex <==

\subsubsection{Proof of Lemma X}


For a policy $\pi^1$, we denote the space of optimal responses by $\Pi_2 (\pi^1)$ and let $\pi^*(\pi^1) \in \optPi_2(\pi^1)$ denote a fixed optimal response to $\pi^1$. An $\varepsilon$-greedy policy given $\pi^1$ is then defined as
\begin{align*}
    \pi^2_\varepsilon (s, \pi^1) =
    \begin{cases}
    \pi^*(s, \pi^1) & w.p.\ 1-\varepsilon \\
    \mathcal{U}(A_2) & w.p.\ \varepsilon,
    \end{cases}
\end{align*}
where $\varepsilon \in [0,1]$ and $\mathcal{U}(A_2)$ is the uniform distribution over $A_2$. We define the optimal value function $V^*$ as
\begin{align*}
    V^*(s) \defn \sup_{\pi^1} V_{\pi^1, \pi^2_\varepsilon(\pi^1)}(s) \quad \forall s \in \S,
\end{align*}
where we want to emphasise that the supremum is taken separably for each $s \in \S$. In particular, Theorem \ref{lemma:no_dominating_policy} tells us that for some classes of responses, e.g.\ $\bolPi_2$, there may not exists a policy $\pi^1$ such that $V_{\pi^1, \pi^2_\varepsilon(\pi^1)} (s) = V^*(s)$ for all $s \in \S$. 

The problem of planning with an agent that responds with $\varepsilon$-greedy policies is similar to the setting considered by \cite{dimitrakakis2017multi} in the sense that $\A_2$ plans with the original transition kernel $\trans$ (by computing $\pi^*(\pi^1)$), whereas $\A_1$ plans with the ``correct'' transition kernel
\begin{align*}
    \trans_\varepsilon(s' \mid s, a, b) \defn \varepsilon \trans (s' \mid s, a, \mathcal{U}(A_2)) + (1-\varepsilon) \trans (s' \mid s, a, b).
\end{align*} 
In particular, note that $\varepsilon \trans(s' \mid s, a, \mathcal{U}(A_2))$ is independent of the choice of $b$. 

We define the following two operators on the normed vector space $\mathcal{V} = \{ V: \S \to \Reals \colon \| V\|_{\infty} < \infty\}$ equipped with the supremum norm $\lVert \cdot \rVert_{\infty}$
\begin{align*}
    T_{\pi^1}V(s) & = \max_{b} \r(s) + \gamma \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) V(s') \\
    %& = \varepsilon \big(\r(s) + \gamma \sum_{s'} \trans(s'\mid s, \pi^1, \mathcal{U}(A_2)) V(s') \big) + (1-\varepsilon) \max_b \big( \r(s) + \gamma \sum_{s'} \trans(s'\mid s, \pi^1, b) V(s')\big)
    T V(s) & = \max_a \max_b \r(s) + \gamma \sum_{s'} \trans_{\varepsilon} (s' \mid s, a, b) V(s').
\end{align*}
To show that a dominating commitment strategy always exists, we will need that $T_{\pi^1}$ and $T$ are $\gamma$-contractions w.r.t.\ $\lVert \cdot \rVert_{\infty}$. 

\begin{lemma}
The operator $T_{\pi^1}$ is a $\gamma$-contraction on $(\mathcal{V}, \lVert \cdot \rVert_{\infty})$ with unique fix point $V_{\pi^1, \pi^2_\varepsilon(\pi^1)}$. 
\end{lemma}
\begin{proof}
Note that for any two bounded functions $f, g: X \to \Reals$, the following standard inequality holds 
\begin{align}\label{equation:supremum_inequality}
    |\sup_{x \in X} f(x) - \sup_{x \in X} g(x)| \leq \sup_{x \in X} | f(x) - g(x) |.
\end{align}
For any $\pi^1$, we then obtain
\begin{align*}
    \lVert T_{\pi^1} V - T_{\pi^1} U \rVert_{\infty} & = \gamma \sup_{s} | \max_{b} \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) V(s') - \max_{b} \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) U(s') | \\
    & \overset{\eqref{equation:supremum_inequality}}{\leq} \gamma \sup_{s} \max_{b} | \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) (V(s') - U(s'))|\\ 
    % & \leq \gamma \sup_{s} \max_b \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) |V(s')- U(s')|  \\
    & \leq \gamma \sup_s \max_b \sum_{s'} \trans_{\varepsilon} (s' \mid s, \pi^1, b) \lVert V - U \rVert_{\infty} \\
    & = \gamma \lVert V - U \rVert_{\infty}.
\end{align*}
Thus, $T_{\pi^1}$ is a $\gamma$-contraction on $(\mathcal{V}, \lVert \cdot\rVert_{\infty})$. 
In the same vein, by applying equation \eqref{equation:supremum_inequality} to the maximisation $\max_{a} \max_{b}$, we get
\begin{align*}
    \lVert T V - T U \rVert_{\infty} & \leq \gamma \sup_s \max_a \max_b \sum_{s'} \trans_{\varepsilon} (s' \mid s, a, b) \lVert V- U\rVert_{\infty} = \gamma \lVert V - U \rVert_{\infty}.
\end{align*}
Hence, $T$ is a $\gamma$-contractions on $(\mathcal{V}, \lVert \cdot\rVert_{\infty})$. 
\end{proof}


\textcolor{purple}{Need to show that $V_{\pi^1, \pi^2_\varepsilon(\pi^1)}$ is a fix point of $T_{\pi^1}$}

\begin{proof}[\textbf{Proof of Lemma \ref{lemma:value_iteration_for_epsilon}}]
The following proof holds for a possibly infinite state space $\S$ and for finite actions spaces $A_1$ and $A_2$.\footnote{The extension to infinite actions spaces requires an additional continuity assumption to guarantee the existence of a greedy policy. (I think)} If not differently specified, let $s, s' \in \S$, $a \in A_1$ and $b \in A_2$. 





Let $s \in S$. By definition of $V^*$, we have $V_{\pi^1, \pi^2_\varepsilon(\pi^1)} (s) \leq V^*(s)$ for any $\pi^1$. Applying the operator $T_{\pi^1}$ on both sides, we then get $V_{\pi^1, \pi^2_\varepsilon(\pi^1)}(s) \leq T_{\pi^1} V^*$, where we have used that $\pi^1$ is the (unique) fix point of $T_{\pi^1}$. Taking the supremum over $\pi^1$ on both sides, it then follows that 
\begin{align*}
    V^*(s) = \sup_{\pi^1} V_{\pi^1, \pi^2_\varepsilon(\pi^1)} (s) \leq \sup_{\pi^1} T_{\pi^1} V^*(s) = TV^*(s),
\end{align*}
where the last equality holds by definition of $T_{\pi^1}$ and $T$. Crucially, note that taking the supremum over all $s \in \S$, i.e.\ $\sup_{\pi^1} V_{\pi^1, \pi^2_{\varepsilon}(\pi^1)}$, would not be well-defined as we do not know whether a dominating policy $\pi^1$ maximising $V_{\pi^1, \pi^2_{\varepsilon}(\pi^1)}(s)$ for all $s\in \S$ exists. However, we are can establish the above relation for each $s \in \S$ separably.

We now define the policy $\pi^1$ as the policy such that $T_{\pi^1}V^* = T V^*$, i.e.\ for $s \in \S$
\begin{align*}
    \pi^1(s) = \argmax_{a} \max_b \r(s) + \gamma \sum_{s'} \trans_{\varepsilon} (s' \mid s, a, b) V^*(s').
\end{align*}
Note that $\pi^1$ is well-defined. In particular, while the $\varepsilon$-greedy response $\pi^2_{\varepsilon}$ depends on the complete policy $\pi^1$, we defined the operators $T_{\pi^1}$ and $T$ such that $\A_2$'s response is expressed using the term $\max_b$.

It follows that $T_{\pi^1} V^* \succeq V^*$ 
\vspace{2cm}

\end{proof}

==> sections/proofs.tex <==
\section{Proofs}

\begin{proof}[Proof of Lemma~\ref{lem:maximin_zero}]
For simplicity of exposition, we assume here that the posterior $\P$ is discrete. Now, as the value function is linear in rewards, we have 
\begin{align*}
    \min_{\pi} \bayesregret_\P (\trans, \pi) = \bayesregret_\P (\trans, \pi_{\bar \r, \trans}),
\end{align*}
where $\pi_{\bar \r, \trans}$ is the optimal policy w.r.t.\ the posterior mean $\bar \r = \E_{\r \sim \P}[\r]$ and the transition function $\trans$. If $\max_{\trans \in \Trans} \min_{\pi \in \Pi} \bayesregret_\P (\trans, \pi) = 0$, it then follows that $\max_{\trans \in \Trans} \bayesregret_\P (\trans, \pi_{\bar \r, \trans}) = 0$, i.e.\ $\val_{\r, \trans}^* = \val_{\r, \trans}^{\pi_{\bar \r, \trans}}$ for all $\r \in \supp(\P)$ and $\trans \in \Trans$. This must imply that $\val_{\truereward, \trans}^* = \val_{\truereward, \trans}^{\pi_{\bar \r, \trans}}$ for all $\trans \in \Trans$. In other words, $\bar \r$ is optimal for all $\trans \in \Trans$ (under the initial state distribution $\omega$). 
\end{proof}


\iffalse
Fix $\trans$ and $\P$. Let $\pi^E_{\trans}$ denote the observed expert policy in $\trans$.  
Define the sets 
\begin{equation*}
    \cB_\trans(\pi) = \{ \r: \pi_{\r, \trans} = \pi\} 
\end{equation*}
and let $\cB_\trans^* = \cB_\trans(\pi_{\truereward, \trans})$.
Let $\bar \pi_\trans = \min_\pi \bayesregret_{\P}(\trans, \pi)$ and define $\cR^+(T) = \{ \r : \val_{\r, \trans}^* > \val_{\r, \trans}^{\bar \pi_\trans} \}$. 

Now, for any $\r \in \cR^+(T)$, we either have a) $\r \in \cB^*_\trans$, or b) $\r \not \in \cB^*_\trans$. Note that we can determine whether a) and b) holds by simply comparing $\pi_{\r, \trans}$ with $\pi_\trans^E$. 

If a) holds, then we have $\val_{\r, \trans}^{\pi^E_\trans} = \val_{\r, \trans}^* > \val_{\r, \trans}^{\bar \pi_{\trans}}$, which implies that $\bar \pi_\trans \neq \pi_{\trans}^E $. As a consequence, for at least one $\r' \in \supp(\P)$, it must hold that $\pi_{\r', \trans} \neq \pi_\trans^E$, which can easily be checked via contradiction. Thus, the expert policy $\pi_\trans^E$ is suboptimal under $\r'$ and $\trans$ so that any reward function in the equivalence class $\cB_\trans (\pi_{\r', \trans})$ cannot be in the support of $\P$ anymore after observing $\pi_\trans^E$. 


If b) holds, it follows that $\pi_{\r, \trans} \neq \pi_\trans^E$, which implies that $\pi_\trans^E$ is suboptimal under $\r$. As a result, we have that any reward function in $\cB_\trans(\pi_{\r, \trans})$ cannot be in the support of $\P$ after observing $\pi_\trans^E$.




On the other hand, if the objective is nonzero given a distribution $\P$ (as will be typically the case), we can ...


In general, we cannot achieve zero maximin Bayesian regret 

As a analytical justification of the Bayesian regret objective in addition to our empirical evaluation, we derive that 

\begin{lemma}
    Suppose that the optimal policy w.r.t.\ any $\r$ and $\trans$ is unique. Suppose that the expert is optimal and we observe the full expert policy. Let the posterior in round $k$ be denoted by $\P_k$ and let $\trans = \max_{\trans} \min_{\pi} \bayesregret_{\P_k} (\trans, \pi)$. Then, we have $\min_{\pi} \bayesregret_{\P_{k+1}}(\trans, \pi) < \min_{\pi} \bayesregret_{\P_k} (\trans, \pi)$ or $\max_T \min_\pi \bayesregret_{\P_k}(\trans, \pi) = 0$.  
\end{lemma} 




\begin{lemma}
    (If the expert is optimal and we see the whole policy) Choosing transition functions according to the Bayesian regret in fact minimises the Bayesian regret of the learner (w.r.t.\ $\P_k$). 
    
    As a result, as $k \to \infty$, the Bayesian regret will be zero. 
    
    This in turns means that the learner will be optimal on all transition functions in $\Trans$. 
    
    If the learner is optimal on all transition functions in $\Trans$, then it has this ... guarantee on similar transition functions. 
    
    % Note that we do not address the sample-complexity and assume availability of the expert policy for convenience. The sample-complexity when only observing trajectories heavily depends on the IRL algorithm used. 
\end{lemma}

\fi

==> sections/tables/normalized_scores_with_base.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{10pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.4} % Default value: 1
\resizebox{\linewidth}{!}{%
\begin{tabular}{L{0.08\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}|C{0.075\textwidth}}
%\cline{2-16}
\multicolumn{1}{C{0.08\textwidth}|}{}&
  \multicolumn{3}{C{0.32\textwidth}|}{Continuous maze} &
  \multicolumn{3}{C{0.32\textwidth}|}{Hopper} &
  \multicolumn{3}{C{0.32\textwidth}|}{HalfCheetah} &
  \multicolumn{3}{C{0.32\textwidth}}{Swimmer} \\ \cline{2-13}
\multicolumn{1}{C{0.08\textwidth}|}{} &
  \multicolumn{1}{C{0.075\textwidth}|}{Base} &
  \multicolumn{1}{C{0.075\textwidth}|}{Demo} &
  \multicolumn{1}{C{0.075\textwidth}|}{Test} &
  \multicolumn{1}{C{0.075\textwidth}|}{Base} &
  \multicolumn{1}{C{0.075\textwidth}|}{Demo} &
  \multicolumn{1}{C{0.075\textwidth}|}{Test} &
  \multicolumn{1}{C{0.075\textwidth}|}{Base} &
  \multicolumn{1}{C{0.075\textwidth}|}{Demo} &
  \multicolumn{1}{C{0.075\textwidth}|}{Test} &
  \multicolumn{1}{C{0.075\textwidth}|}{Base} &
  \multicolumn{1}{C{0.075\textwidth}|}{Demo} &
  \multicolumn{1}{C{0.075\textwidth}}{Test} \\ \midrule
\multicolumn{1}{L{0.09\textwidth}|}{$\edairl$} &
  81±23 &
  \textbf{68±08} &
  \textbf{71±05} &
  
  47±27 &
  \textbf{63±22} &
  52±13 &
  
  62±78 &
  \textbf{57±39} &
  \textbf{62±53} &

  78±52 &
  80±51 &
  69±37 \\ %\cdashline{1-13}
\multicolumn{1}{L{0.08\textwidth}|}{$\drairl$} &
  82±23 &
  52±16 &
  53±27 &
  
  31±14 &
  59±18 &
  \textbf{56±13} &

  74±63 &
  51±32 &
  46±39 &
    
  54±28 &
  45±13 &
  53±17 \\ \cdashline{1-13}
\multicolumn{1}{L{0.08\textwidth}|}{$\airl$} &
  59±28 &
  33±21 &
  52±15 &
  
  66±31 &
  38±08 &
  34±13 &

  \textbf{145±32} &
  42±12 &
  22±13 &
  
  61±40 &
  40±30 &
  44±24 \\ %\cdashline{1-13}
  &&&&&&&&&&&& \\
\multicolumn{1}{L{0.08\textwidth}|}{$\bc$} &
  \textbf{107±00} &
  11±01 &
  22±00 &
  
  67±13 &
  36±03 &
  31±03 &
  
  84±01 &
  43±01 &
  21±04 &

  \textbf{127±01} &
  \textbf{124±02} &
  \textbf{130±02} \\ %\hline
\multicolumn{1}{L{0.08\textwidth}|}{$\gail$} &
  105±01 &
  20±11 &
  17±03 &
  
  \textbf{107±05} &
  45±05 &
  39±03 &
  
  107±06 &
  39±03 &
  23±02 &

  127±01 &
  111±01 &
  110±02 \\ %\cdashline{1-13}
\multicolumn{1}{L{0.08\textwidth}|}{$\rime$} &
  ?±? &
  ?±? &
  ?±? &
  
  ?±? &
  ?±? &
  ?±? &

  ?±? &
  ?±? &
  ?±? &

  ?±? &
  ?±? &
  ?±? \\
\end{tabular}%
}
\vspace{7px}
\caption{\label{tab:normalized_returns_with_base} Average normalized returns of the algorithms on the base environment, demo set, and test set (averaged over 10 runs for MuJoCo and 5 runs for the maze task). 100 indicates expert performance, whereas 0 indicates the performance of a random policy. 
\vspace{-.5cm}}
\end{table*}

==> sections/theory.tex <==

\section{Theoretical Questions:} 


% \begin{theorem}
% Suppose that the posterior $\P(\cdot \mid \data)$ satisfies $\min_{\trans \in \Trans} \max_{\pi \in \Pi} \bayesregret_\P (\trans, \pi) = 0$. Then, 
% \begin{enumerate}
%     \item $\bar \r$ induces an optimal policy in $(\S, \A,  \trans, \truereward, \gamma)$ for all $\trans \in \Trans$
%     \item $\mathrm{Mixture}(\Trans)$ 
% \end{enumerate}
% \end{theorem} 

We can define the \emph{reward loss} of $\r$ on $\trans$ as $ \mathscr{L}_\trans (\r) = \val^*_{\truereward, \trans} - \val_{\truereward, \trans}^{\pi_{\r, \trans}}$. This is equal to $\ell_{\truereward} (\trans, \pi_{\r, \trans})$. This can be understood as the loss of optimising for rewards $\r$ instead of the true rewards $\truereward$ on $\trans$.  

\begin{lemma}[Generalisability of Optimal Rewards]
Suppose that $\r$ is optimal for $\trans_1$ and $\trans_2$. For $\trans \equiv w \trans_1 + (1-w) \trans_2$, we have 
\begin{equation*}
    \mathscr{L}_T(\r) \leq ...
\end{equation*}

\end{lemma}

Claim: If the stationary state distribution w.r.t. $(\pi_1, T_1)$ and $(\pi_2, T_2)$ have the same support, then the stationary state distribution of $(\pi_{R, T}, T_w)$ has the same support as well.

\begin{lemma}[Generalisability of Optimal Rewards with Optimal Demonstrator]
Suppose that $\r$ is optimal for $\trans_1$ and $\trans_2$ \emph{and} that we observed the optimal policies $\pi_{\truereward, \trans_1}$ and $\pi_{\truereward, \trans_2}$. For $\trans \equiv w \trans_1 + (1-w) \trans_2$, we get a slightly refined bound of 
\begin{equation*}
    \mathscr{L}_T(\r) \leq ...
\end{equation*}
\end{lemma}


\subsection{Rewards are generally not transferable}
\begin{lemma}[Lower Bound on Generalisability]
There exist $(\S, \A, \trans, \truereward, \gamma)$ such that a reward function $\r$ induces an optimal policy w.r.t.\ $\trans$, but there exists $\trans_\varepsilon$ with $\lVert \trans - \trans_{\varepsilon} \rVert \leq \varepsilon$ such that  
$$\mathscr{L}_{\trans_{\varepsilon}}(\r) \geq \frac{\max_s \truereward(s)}{1-\gamma} ...$$
\end{lemma}
----

% Rewards learned from a single environment can be arbitrarily bad on an $\varepsilon$-far away environment. 


\section*{Notation}

\begin{itemize}
    \item $\pi_{\r, \trans}$ --- \emph{optimal} policy in MDP $(\S, \A, \trans, \r, \gamma)$
    \item $\val^\pi_{\r, \trans}$ --- value function under initial state distribution $\omega$ and $\pi, \r, \trans$
    \item $\truereward$ --- true reward function
    \item $\r$ --- generic reward function 
\end{itemize}

\newpage 


\begin{enumerate}

    \item Can we show something w.r.t.\ the robustness of rewards learned from a single environment? 
    
    Something of the lines of: Minor deviations in the environment dynamics can make the reward function break. 
    
    Similarly, can we show that a demonstration in another environment can prevent this breaking? 
    
    \item Can we show something addressing the sample-efficiency of learning from a single env vs multiple env?
    
\end{enumerate}

\subsection{Limitations of Learning from Single Environment}

(IRL and the identifiability of rewards \cite{kim2021reward, cao2021identifiability}) 

\subsection{Power of Learning from Multiple Environments} 

Check \cite{cao2021identifiability} for their result on demonstrations with different discount factors. 


Q: If a reward function is optimal on $\trans_1$ and $\trans_2$, what is the guarantee on mixtures $w \trans_1 + (1-w) \trans_2$?

Based on \cite{viano2021robust}, we possibly get (actually not what we are interested in)
$$| \val_\trans - \val_{\trans'}| \leq \frac{\gamma}{1-\gamma} \min_{\trans \in \Trans} \textrm{dist}(\trans, \trans').$$ 

For some $\r$, suppose that $\pi^*_{\r, \trans}$ is optimal $\forall \trans \in \Trans$. For some other transition function $\trans'$ we are interested in the quantity $|\val_{\truereward, \trans'}^* - \val_{\truereward, \trans'}^{\pi^*_{\r, \trans'}}|$. 
Do we have $\val^{\pi_{\r, \trans'}}_{\truereward, \trans'} \geq \val^{\pi_{\r, \trans}}_{\truereward, \trans'}$ for all $\trans \in \Trans$? In general, probably no. However, when $\trans'$ is a mixture, probably yes? 

We want a statement like: "If $\r$ is optimal on this set of MDPs, then we know that on its mixtures $\r$ is guaranteed to be at least this good." 

\subsection{Hypotheses}
It will be interesting to consider the following hypotheses: 
\begin{itemize}
    \item[a)] \emph{The more influence the expert has on transitions, the more informative the demonstrations. }
    
    \item[b)] \emph{Environments that are difficult to solve (while being solvable) are more informative. }  
    
    \item[c)] \emph{A reward function learned from a sequence of designed environments generalises better. }
    
\end{itemize}
a) In what sense more informative?

c) That is, not only can we be more certain about the reward function, but the learned reward function yields robust policies that transfer well to all environments in $\Param$. Thus, Curriculum Learning for IRL could also yield more robust reward functions (in the sense of transferability to similar environments). This is generally the goal as we do not simply wish to learn a reward which allows us to imitate agents in the current environment, but which allows us to predict their actions in other settings. 


